Roots of $L$-functions of characters over function fields, generic linear independence and biases

We first show joint uniform distribution of values of Kloosterman sums or Birch sums among all extensions of a finite field $\mathbb{F}_q$, for almost all couples of arguments in $\mathbb{F}_q^\times$, as well as lower bounds on differences. Using similar ideas, we then study the biases in the distribution of generalized angles of Gaussian primes over function fields and primes in short intervals over function fields, following recent works of Rudnick--Waxman and Keating--Rudnick, building on cohomological interpretations and determinations of monodromy groups by Katz. Our results are based on generic linear independence of Frobenius eigenvalues of $\ell$-adic representations, that we obtain from integral monodromy information via the strategy of Kowalski, which combines his large sieve for Frobenius with a method of Girstmair. An extension of the large sieve is given to handle wild ramification of sheaves on varieties.

==> commands.tex <==
%auto-ignore

\newcommand{\declarecommand}[1]{\providecommand{#1}{}\renewcommand{#1}}

% Miscellaneous
\newcommand{\cdotarg}{\, \cdot \,}
\newcommand{\co}{\backslash}
\newcommand{\normal}{\mathrel{\unlhd}}
\newcommand{\dia}[1]{\langle#1\rangle}
\newcommand{\mtu}{\,--\,}
\newcommand{\closure}{\overline}
\newcommand*\elide{\textup{[\,\dots]}}
\newcommand{\sump}{\sideset{}{'}\sum}

% Floor/Ceil
\providecommand{\ceil}[1]{\left \lceil #1 \right \rceil }
\providecommand{\floor}[1]{\left \lfloor #1 \right \rfloor }

%Matrix groups and Lie algebras
\newcommand{\GL}{\operatorname{GL}}
\newcommand{\GU}{\operatorname{GU}}
\newcommand{\PGL}{\operatorname{PGL}}
\newcommand{\SL}{\operatorname{SL}}
\declarecommand{\sl}{\mathfrak{sl}}
\newcommand{\SO}{\operatorname{SO}}
\newcommand{\Spin}{\operatorname{Spin}}
\newcommand{\so}{\mathfrak{so}}
\declarecommand{\O}{\operatorname{O}}
\newcommand{\GO}{\operatorname{GO}}
\newcommand{\PSL}{\operatorname{PSL}}
\newcommand{\SU}{\operatorname{SU}}
\newcommand{\Sp}{\operatorname{Sp}}
\newcommand{\GSp}{\operatorname{GSp}}
\declarecommand{\sp}{\mathfrak{sp}}
\newcommand{\PSp}{\operatorname{PSp}}
\newcommand{\PSO}{\operatorname{PSO}}
\newcommand{\USp}{\operatorname{USp}}
\newcommand{\PSU}{\operatorname{PSU}}

% Blackboard
\newcommand{\A}{\mathbb{A}}
\declarecommand{\P}{\mathbb{P}}
\newcommand{\C}{\mathbb{C}}
\newcommand{\E}{\mathbb{E}}
\newcommand{\F}{\mathbb{F}}
\newcommand{\G}{\mathbb{G}}
\newcommand{\HI}{\mathbb{H}}
\newcommand{\N}{\mathbb{N}}
\newcommand{\Q}{\mathbb{Q}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\Sb}{\mathbb{S}}
\newcommand{\T}{\mathbb{T}}
\newcommand{\W}{\mathbb{W}}
\newcommand{\Z}{\mathbb{Z}}

% Kloosterman
\newcommand{\Kl}{\operatorname{Kl}}
\newcommand{\Klc}{\mathcal{K}l}

% Operators
\declarecommand{\Hom}{\operatorname{Hom}}
\newcommand{\End}{\operatorname{End}}
\newcommand{\Ei}{\operatorname{Ei}}
\newcommand{\Aut}{\operatorname{Aut}}
\newcommand{\Tor}{\operatorname{Tor}}
\newcommand{\arctanh}{\operatorname{arctanh}}
\newcommand{\Inn}{\operatorname{Inn}}
\newcommand{\Out}{\operatorname{Out}}
\newcommand{\Graph}{\operatorname{Graph}}
\newcommand{\genus}{\operatorname{genus}}
\newcommand{\Jac}{\operatorname{Jac}}
\newcommand{\rad}{\operatorname{rad}}
\newcommand{\diag}{\operatorname{diag}}
\newcommand{\Mat}{\operatorname{Mat}}
\newcommand{\Ind}{\operatorname{Ind}}
\newcommand{\Id}{\operatorname{Id}}
\newcommand{\id}{\operatorname{id}}
\newcommand{\Li}{\operatorname{Li}}
\newcommand{\ord}{\operatorname{ord}}
\newcommand{\codim}{\operatorname{codim}}
\newcommand{\cond}{\operatorname{cond}}
\newcommand{\sgn}{\operatorname{sgn}}
\newcommand{\Sing}{\operatorname{Sing}}
\newcommand{\Swan}{\operatorname{Swan}}
\newcommand{\Stab}{\operatorname{Stab}}
\newcommand{\Isom}{\operatorname{Isom}}
\newcommand{\Lie}{\operatorname{Lie}}
\newcommand{\dropp}{\operatorname{drop}}
\newcommand{\trdeg}{\operatorname{trdeg}}
\newcommand{\der}{\mathrm{der}}
\newcommand{\lcm}{\operatorname{lcm}}
\newcommand{\height}{\operatorname{height}}
\newcommand{\im}{\operatorname{im}}
\newcommand{\car}{\operatorname{char}}
\newcommand{\charpol}{\operatorname{charpol}}
\newcommand{\inv}{^{-1}}
\newcommand{\disc}{\operatorname{disc}}
\newcommand{\lspan}{\operatorname{span }}
\newcommand{\fix}{\operatorname{fix}}
\newcommand{\tr}{\operatorname{tr}}
\newcommand{\Fr}{\operatorname{Fr}}
\newcommand{\ch}{\operatorname{ch}}
\newcommand{\Gal}{\operatorname{Gal}}
\newcommand{\Sym}{\operatorname{Sym}}
\newcommand{\Symm}{\operatorname{Symm}}
\newcommand{\Twists}{\operatorname{Twists}}
\newcommand{\Alt}{\operatorname{Alt}}
\newcommand{\Pic}{\operatorname{Pic}}
\newcommand{\Div}{\operatorname{Div}}
\declarecommand{\Re}{\operatorname{Re}}
\newcommand{\res}{\operatorname{res}}
\declarecommand{\Im}{\operatorname{Im}}
\declarecommand{\Spec}{\operatorname{Spec}}
\declarecommand{\Proj}{\operatorname{Proj}}
\newcommand{\rank}{\operatorname{rank}}
\newcommand{\rk}{\operatorname{rk}}
\declarecommand{\supp}{\operatorname{supp}}
\newcommand{\Frob}{\operatorname{Frob}}
\newcommand{\FT}{\operatorname{FT}}
\newcommand{\mult}{\operatorname{mult}}
\newcommand{\orb}{\operatorname{orb}}
\newcommand{\Std}{\operatorname{Std}}
\newcommand{\Cov}{\operatorname{Cov}}
\declarecommand{\Var}{\operatorname{Var}}
\newcommand{\erf}{\operatorname{erf}}
\newcommand{\erfc}{\operatorname{erfc}}
\newcommand{\NS}{\operatorname{NS}}

\newcommand{\No}{\operatorname{N}} % Normalizer
\newcommand{\sep}{\mathrm{sep}}
\newcommand{\hol}{\mathrm{hol}}
\newcommand{\alg}{\mathrm{alg}}
\declarecommand{\div}{\mathrm{div}}
\declarecommand{\pdiv}{\mathrm{pdiv}}
\newcommand{\prob}{\mathrm{prob}}
\newcommand{\geom}{\mathrm{geom}}
\declarecommand{\semisimple}{\mathrm{ss}}
\newcommand{\arith}{\mathrm{arith}}
\newcommand{\new}{\mathrm{new}}
\newcommand{\old}{\mathrm{old}}

% Fraktur
\newcommand{\af}{\mathfrak{a}}
%\declarecommand{\bf}{\mathfrak{b}}
\newcommand{\cf}{\mathfrak{c}}
\newcommand{\gf}{\mathfrak{g}}
\newcommand{\pf}{\mathfrak{p}}
\newcommand{\qf}{\mathfrak{q}}
\newcommand{\lf}{\mathfrak{l}}
\newcommand{\Pf}{\mathfrak{P}}
\newcommand{\mf}{\mathfrak{m}}
\newcommand{\Mf}{\mathfrak{M}}
\newcommand{\Sf}{\mathfrak{S}}

% Cal
\newcommand{\Ac}{\mathcal{A}}
\newcommand{\Bc}{\mathcal{B}}
\newcommand{\Cc}{\mathcal{C}}
\newcommand{\Ec}{\mathcal{E}}
\newcommand{\Fc}{\mathcal{F}}
\newcommand{\Gc}{\mathcal{G}}
\newcommand{\Hc}{\mathcal{H}}
\newcommand{\Ic}{\mathcal{I}}
\newcommand{\Jc}{\mathcal{J}}
\newcommand{\Kc}{\mathcal{K}}
\newcommand{\Lc}{\mathcal{L}}
\declarecommand{\Mc}{\mathcal{M}}
\newcommand{\Nc}{\mathcal{N}}
\newcommand{\Oc}{\mathcal{O}}
\newcommand{\Pc}{\mathcal{P}}
\newcommand{\Rc}{\mathcal{R}}
\newcommand{\Sc}{\mathcal{S}}
\newcommand{\Tc}{\mathcal{T}}
\newcommand{\Cl}{\mathcal{C}l}


%Legendre symbol
\newcommand{\legendre}[2]{\left(\frac{#1}{#2}\right)}
\newcommand{\dlegendre}[2]{\left(\frac{#1}{#2}\right)}

%Bold symbols and letters
\declarecommand{\bs}{\boldsymbol}
\newcommand{\Gb}{\bm{G}}
\newcommand{\Tb}{\bm{T}}
\newcommand{\Vb}{\bm{V}}

% Averages
\newcommand{\aver}[3]{\frac{1}{#3}\sum_{#1\in #2}}
\newcommand{\averC}[2]{\aver{#1}{#2}{|#2|}}

%TODO
\newcommand{\TODO}[1]{[{\color{red}\sffamily\textbf{todo:} #1}]}
\newcommand{\later}[1]{[{\color{black}\sffamily\small\textbf{later:} #1}]}
\newenvironment{TODOb}{\color{red}\sffamily{\begin{center}\rule{0.4\textwidth}{0.5pt}\textbf{TODO}\rule{0.4\textwidth}{0.5pt}\end{center}}}{\begin{center}\rule{\textwidth}{0.5pt}\end{center}}
\definecolor{light-gray}{gray}{0.5}
\newenvironment{laterb}{\color{light-gray}\sffamily}{}

%http://tex.stackexchange.com/questions/58141/equations-inside-enumerate-aligned-on-items-number
\newcommand\Item[1][]{%
  \ifx\relax#1\relax  \item \else \item[#1] \fi
  \abovedisplayskip=0pt\abovedisplayshortskip=0pt~\vspace*{-\baselineskip}}

%https://tex.stackexchange.com/questions/39221/removing-extra-space-with-pmod-command
\makeatletter
\let\@@pmod\pmod
\DeclareRobustCommand{\pmod}{\@ifstar\@pmods\@@pmod}
\def\@pmods#1{\mkern4mu({\operator@font mod}\mkern 6mu#1)}
\makeatother

%http://tex.stackexchange.com/questions/4302/prettiest-way-to-typeset-c-cplusplus
\newcommand{\CC}{C\nolinebreak\hspace{-.05em}\raisebox{.4ex}{\tiny\bf +}\nolinebreak\hspace{-.10em}\raisebox{.4ex}{\tiny\bf +}}
\def\CC{{C\nolinebreak[4]\hspace{-.05em}\raisebox{.4ex}{\tiny\bf ++}}}

\newcommand{\inlinelabel}[1]{\hfill\refstepcounter{equation}\label{#1}\textup{(\theequation)}}


\newcommand\blfootnote[1]{%
  \begingroup
  \renewcommand\thefootnote{}\footnote{#1}%
  \addtocounter{footnote}{-1}%
  \endgroup
}

\newcommand{\mailto}[1]{\href{mailto:#1}{#1}}

%https://tex.stackexchange.com/questions/169907/how-to-typeset-the-house-of-an-algebraic-number
\makeatletter
\newcommand*{\house}[1]{%
  \mathord{%
    \mathpalette\@house{#1}%
  }%
}
\newcommand*{\@house}[2]{%
  % #1: math style
  % #2: expression that gets the "house"
  % get the line width of `\overline' in the current math font size
  \dimen@=\fontdimen8 %
      \ifx#1\scriptscriptstyle\scriptscriptfont
      \else\ifx#1\scriptstyle\scriptfont
      \else\textfont\fi\fi
      3 %
  \sbox0{%
    $#1%
      \vrule width\dimen@\relax
      \overline{%
        \kern2\dimen@
        \begingroup % to keep changes of \dimen@ in #2 local
          #2%
        \endgroup
        \kern2\dimen@
      }%
      \vrule width\dimen@\relax
      \mathsurround=1.5\dimen@ % outside margin
    $%
  }%
  % TeX adds an empty space above `\overline', it needs to be
  % removed to get the correct height for the `\vrule's
  \ht0=\dimexpr\ht0-\dimen@\relax
  \dp0=\dimexpr\dp0+2\dimen@\relax
  \vbox{%
    \kern\dimen@ % reinsert previously removed space
    \copy0 %
  }%
}

==> enumerate.tex <==
%auto-ignore
\renewcommand{\labelitemi}{--}

\usepackage[inline,shortlabels]{enumitem} % Call after babel
%\setenumerate{itemsep=0mm,topsep=0.1cm}
\setenumerate[1]{label={(\arabic*)}}

==> hyperref.tex <==
%auto-ignore
\usepackage[lowtilde]{url}
\usepackage[linktocpage,bookmarksdepth=2]{hyperref}
\hypersetup{
%    hidelinks,
     colorlinks,
     linkcolor=green,
     citecolor=green,
     urlcolor=blue
}
\urlstyle{rm}

==> packages.tex <==
%auto-ignore
\usepackage{etex}
\usepackage{amsthm}
\usepackage{amssymb}
\usepackage{amsmath}
\usepackage{mathtools}
\usepackage{mathabx}
\usepackage{multirow}
\usepackage{graphicx}
%\usepackage{grffile}
\usepackage{pstricks}
\usepackage{pst-plot}
\usepackage{pstricks-add}
\usepackage{bm}
\usepackage{fp}
\usepackage{multido}
\usepackage{subfig} %conflicts with tocloft
\psset{algebraic=true}
\usepackage[all]{xy}
\usepackage{subfiles}
\usepackage{multicol}

\usepackage{color}
\definecolor{vlightgray}{gray}{0.95}

% Adjust bibliography spacing and font size
\ifarxiv
  % %For arxiv submissions
  \let\OLDthebibliography\thebibliography
  \renewcommand\thebibliography[1]{
  \OLDthebibliography{#1}
  \setlength{\parskip}{0pt}
  \setlength{\itemsep}{0.3cm}
  }
  \renewcommand{\bibliofont}{\small}
\else
  \ifbiblatex
    \usepackage[style=trad-alpha,sorting=nyt]{biblatex}
    \renewcommand*{\bibfont}{\small}
    \setlength\bibitemsep{0.3cm}
  \else
    %With bibtex
    \usepackage{natbib}
    \setlength{\bibsep}{0.3cm}
    %\setcitestyle{authoryear}
    \def\bibfont{\small}
  \fi
\fi
\usepackage[utf8]{inputenc}
\usepackage[T1]{fontenc}

==> pagesize.tex <==
%auto-ignore
\def\@@ptsize{11pt}
\DeclareOption{10pt}{\def\@@ptsize{10pt}}
\DeclareOption{11pt}{\def\@@ptsize{11pt}}
\DeclareOption{12pt}{\def\@@ptsize{12pt}}

==> theorems.tex <==
%auto-ignore
\newcounter{theoscounter}
%\numberwithin{theoscounter}{section}
\newtheoremstyle{thm}{0.4cm}{0.4cm}{\itshape}{}{\bfseries}{.}{.5em}{}
\newtheoremstyle{def}{0.3cm}{0.3cm}{}{}{\scshape}{.}{.5em}{}
\newtheoremstyle{exre}{0.4cm}{0.4cm}{}{}{\itshape}{.}{.5em}{}

\theoremstyle{def}
\let\definition\relax
\newtheorem{definition}[theoscounter]{Definition}
\newtheorem{notation}[theoscounter]{Notation}
\newtheorem{convention}[theoscounter]{Convention}

\theoremstyle{thm}
\newtheorem{theorem}[theoscounter]{Theorem}
\newtheorem*{theorem*}{Theorem}
\newtheorem{proposition}[theoscounter]{Proposition}
\newtheorem*{proposition*}{Proposition}
\newtheorem{corollary}[theoscounter]{Corollary}
\newtheorem*{corollary*}{Corollary}
\newtheorem{claim}[theoscounter]{Claim}
\newtheorem{lemma}[theoscounter]{Lemma}
\newtheorem*{lemma*}{Lemma}

\theoremstyle{exre}
\newtheorem{conjecture}[theoscounter]{Conjecture}
\newtheorem{hypothesis}[theoscounter]{Hypothesis}
\newtheorem{question}[theoscounter]{Question}
\newtheorem*{question*}{Question}
\newtheorem{example}[theoscounter]{Example}
\newtheorem*{example*}{Example}
\newtheorem{examples}[theoscounter]{Examples}
\newtheorem*{examples*}{Examples}
\newtheorem{questions}[theoscounter]{Questions}
\newtheorem{remark}[theoscounter]{Remark}
\newtheorem*{remark*}{Remark}
\newtheorem*{acknowledgements}{Acknowledgements}
\newtheorem{remarks}[theoscounter]{Remarks}
\newtheorem*{remarks*}{Remarks}

%\numberwithin{theoscounter}{section}

